Improving Sparse Word Representations with Distributional Inference for Semantic Composition

Distributional models are derived from co-occurrences in a corpus, where only a small proportion of all possible plausible co-occurrences will be observed. This results in a very sparse vector space, requiring a mechanism for inferring missing knowledge. Most methods face this challenge in ways that render the resulting word representations uninterpretable, with the consequence that semantic composition becomes hard to model. In this paper we explore an alternative which involves explicitly inferring unobserved co-occurrences using the distributional neighbourhood. We show that distributional inference improves sparse word representations on several word similarity benchmarks and demonstrate that our model is competitive with the state-of-the-art for adjective-noun, noun-noun and verb-object compositions while being fully interpretable.

==> future_work.tex <==
In this work we have smoothed the vector space on the basis of PPMI values, but it is possible to smooth the vectors at the co-occurrence count level, and compute PPMI \emph{after} smoothing, which we will explore in future work. A further option is to apply the smoothing operation on the offset vector when composing two lexemes instead of the original vector (or even on both). This has the potential to more precisely enrich the meaning of an offset vector, when already put into context. Futhermore, using the same number of clusters for every word appeared to be to strong a constraint to appropriately handle the polysemous semantics of a word's distributional neighbourhood. Therefore we will investigate tuning the number of clusters on a \emph{per word} basis in future work.
%investigate options in clustering (although clustering was shit in this work, we would like to investigate it further because this appears to be an interesting thing to be doing)
%build an ensemble model by e.g. adding senses from word2vec and WordNet.
%more iterations
